Answer Summarization for Technical Queries: Benchmark and New Approach

Prior studies have demonstrated that approaches to generate an answer summary for a given technical query in Software Question and Answer (SQA) sites are desired. We find that existing approaches are assessed solely through user studies. There is a need for a benchmark with ground truth summaries to complement assessment through user studies. Unfortunately, such a benchmark is non-existent for answer summarization for technical queries from SQA sites. To fill the gap, we manually construct a high-quality benchmark to enable automatic evaluation of answer summarization for technical queries for SQA sites. Using the benchmark, we comprehensively evaluate the performance of existing approaches and find that there is still a big room for improvement. Motivated by the results, we propose a new approach TechSumBot with three key modules:1) Usefulness Ranking module, 2) Centrality Estimation module, and 3) Redundancy Removal module. We evaluate TechSumBot in both automatic (i.e., using our benchmark) and manual (i.e., via a user study) manners. The results from both evaluations consistently demonstrate that TechSumBot outperforms the best performing baseline approaches from both SE and NLP domains by a large margin, i.e., 10.83%-14.90%, 32.75%-36.59%, and 12.61%-17.54%, in terms of ROUGE-1, ROUGE-2, and ROUGE-L on automatic evaluation, and 5.79%-9.23% and 17.03%-17.68%, in terms of average usefulness and diversity score on human evaluation. This highlights that the automatic evaluation of our benchmark can uncover findings similar to the ones found through user studies. More importantly, automatic evaluation has a much lower cost, especially when it is used to assess a new approach. Additionally, we also conducted an ablation study, which demonstrates that each module in TechSumBot contributes to boosting the overall performance of TechSumBot.

==> texUtils.tex <==
\usepackage{xcolor}
\usepackage{enumitem}
\usepackage{amsmath}
\usepackage{eucal}
\usepackage{fancybox}

\usepackage{xcolor}
\usepackage[linesnumbered,ruled,lined]{algorithm2e}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\newcommand{\basicalert}[2]{\fbox{\bfseries\sffamily\scriptsize\color{blue} #1}{\sf\small$\blacktriangleright$\textit{\color{red} #2}$\blacktriangleleft$}}
\newcommand{\bowen}[1]{\basicalert{From Bowen}{#1}}
\newcommand{\cran}[1]{\basicalert{From Cran}{#1}}
\newcommand{\ft}[1]{\basicalert{From Ferdian}{#1}}

% common abbrv
\newcommand{\ie}[0]{i.e.,}
\newcommand{\eg}[0]{e.g.,}
\newcommand{\so}[0]{Stack Overflow}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}


\newcommand{\toolname}[0]{\textsc{TechSumBot}}
\newcommand{\firstmodule}[0]{Usefulness Ranking}
\newcommand{\secondmodule}[0]{Centrality Estimation}
\newcommand{\thirdmodule}[0]{Redundancy Removal}

\newcommand{\se}[0]{software engineering}
\newcommand{\nlp}[0]{NLP community}
\newcommand{\trans}[0]{Transfer learning architecture}
\newcommand{\sent}[0]{our proposed sentence embedding}

\newcommand{\bench}[0]{\textsc{TechSumBench}}


\newcommand{\COMTAG}[2]{{\color{red}Com #1 }{\color{blue}#2}}

